Revisiting DRUP-based Interpolants with CaDiCaL 2.0

We present our implementation of DRUP-based interpolants in CaDiCaL 2.0, and evaluate performance in the bit-level model checker Avy using the Hardware Model Checking Competition benchmarks. CaDiCaL is a state-of-the-art, open-source SAT solver known for its efficiency and flexibility. In its latest release, version 2.0, CaDiCaL introduces a new proof tracer API. This paper presents a tool that leverages this API to implement the DRUP-based algorithm for generating interpolants. By integrating this algorithm into CaDiCaL, we enable its use in model-checking workflows that require interpolants. Our experimental evaluation shows that integrating CaDiCaL with DRUP-based interpolants in Avy results in better performance (both runtime and number of solved instances) when compared to Avy with Glucose as the main SAT solver. Our implementation is publicly available and can be used by the formal methods community to further develop interpolation-based algorithms using the state-of-the-art SAT solver CaDiCaL. Since our implementation uses the Tracer API, it should be maintainable and applicable to future releases of CaDiCaL.

==> Sections/Background.tex <==
\section{Background}
\subsection{Propositional Logic and SAT Solvers}
Propositional logic is a fundamental fragment of First Order Logic (FOL) dealing with propositions that can either be true or false. Generally, propositions are formed using \textit{atomic propositions}, a.k.a Boolean variables, and logical connectives such as $\land, \lor, \neg$, and $\rightarrow$.

SAT solvers are decision procedures developed to determine the satisfiability of a given propositional logic formula that is in \textit{Conjunctive Normal Form} (CNF), a form of propositional logic in which the formula is expressed as a conjunction of one or more clauses, where each clause is a disjunction of literals. A literal is a Boolean variable or its negation. Every propositional logic formula can be efficiently (linearly) transformed into an \textit{equisatisfiable} CNF formula that is linear in size of the original formula via Tseitin transformation~\cite{Tseitin1983}. An equisatisfiable formula is one that is satisfiable if and only if the original formula is satisfiable, ensuring that the transformation preserves the satisfiability of the original formula.

The performance and scalability of SAT solvers have improved tremendously in the past two decades. The continuous advancements in SAT solver technology have led to their widespread adoption in both academia and industry making them essential tools in various fields, including formal verification and model checking.

\subsection{Proofs of Unsatisfiability}
If a propositional logic decision procedure concludes a formula is unsatisfiable, a proof justifying why the formula has no satisfying assignment is required. In literature, such proofs are termed as proofs of unsatisfiability or refutation proofs. While proofs are widely used to certify the correctness of the unsatisfiability result, their applications go beyond that, and the ability to emit proofs of unsatisfiability has become a standard requirement of modern SAT solvers.

Early work on proofs of unsatisfiability focused on \textit{resolution proofs}. The \textit{resolution rule} is a fundamental inference rule used in propositional logic that allows deriving a new clause by resolving two clauses containing complementary literals.
Formally, applying the resolution rule on the clauses $C_1 = (A \lor l)$ and $C_2 = (B \lor \neg l)$, where $A$ and $B$ are clauses (that do not contain complementary literals) and $l$ and $\neg l$ are complementary literals, derives the clause $C_3 = (A \lor B)$. The derived clause $C_3$ is implied by $C_1 \land C_2$, thereby can be added to the CNF while preserving satisfiability. This rule is employed in resolution proofs of unsatisfiability iteratively until the empty clause is derived, indicating that the original formula is unsatisfiable. Resolution proof has become fundamental in formal verification and model checking, and is used in many applications for proof checking, fixing inconsistent specifications, design debugging, formal coverage metrics, unsatisfiable core extraction, abstraction refinement, and interpolation \cite{Interpolation.and.SAT-Based.Model.Checking,10.1007/10722167_15,6679408,DRUPing.for.interpolants}.

On the one hand, once constructed, resolution proofs are easy to process and are efficient to work with. Moreover, most SAT-based model checking approaches that rely on unsatisfiability are based on resolution proofs, making them extremely useful. For instance, one of most important applications of resolution proofs is in reachability analysis~\cite{Biere2018}, where it is used to produce Craig interpolants~\cite{mcmillan2003interpolation}. Given an explicit resolution proof,
there exists a linear-time procedure for generating a Craig interpolant~\cite{Interpolation.and.SAT-Based.Model.Checking,a0092568-8f2a-3f18-91e1-717cd568fea3,10.1007/978-3-642-11319-2_12}.

On the other hand, producing resolution proofs requires substantial modifications to the SAT solver and leads to a significant performance overhead.
% Can drop this since we want to talk only about DRUP
In addition, most processing techniques, that are part of what makes state-of-the-art SAT solvers so efficient, are incompatible - namely, hard to capture with - resolution. As a result, when a resolution proof is required, the model checking algorithm is forced to restrict the SAT solver by disabling these techniques, hindering performance even further.

An alternative proof format is \textit{clausal proofs}~\cite{clausalproofs}, in which proofs are sequences of steps that each modify the current formula by specifying either the deletion of an exiting clause or the addition of a new clause.
In some formats, as in Linear RAT (LRAT) \cite{10.1007/978-3-319-63046-5_14}, hints on clause additions are included.

A clausal proof is \textit{valid} if:
\begin{inparaenum}[(i)]
\item all modifications to the formula can be justified with some specific inference rule (depends on the format, e.g., Reverse Unit Propagation (RUP) as in Delete RUP (DRUP)\cite{Gelder2008VerifyingRP,6679408}, Resolution Asymmetric Tautology (RAT) as in Delete RAT (DRAT) \cite{DBLP:journals/corr/Heule16}); and
\item the proof sequence contains the empty clause, which indicates the formula is unsatisfiable.
\end{inparaenum}

Modern SAT solvers are based on Conflict-Driven Clause Learning (CDCL). During its execution, a CDCL SAT solver learns new clauses to reduce the search space. Additionally, the SAT solver manages the clause database by heuristically deleting learned clauses deemed less helpful. By logging these additions and deletions, CDCL SAT solvers can easily emit clausal proofs with very low overhead~\cite{10.1007/978-3-030-58475-7_25}.

Yet, different clausal proof formats simulate different proof systems; while DRUP format simulates resolution, making it suitable for applications that rely on resolution proofs~\cite{DRUPing.for.interpolants}, DRAT simulates \textit{extended resolution} \cite{DBLP:conf/cade/KieslRH18}.
Extended resolution extends the resolution proof system with the \textit{extension rule}, which allows the introduction of definitions over fresh variables. Compared to simple resolution, extended resolution is exponentially more powerful proof system, with no known exponential lower-bounds on its size. However, it also introduces complexity in how these proofs can be utilized. Unlike DRUP, it is unclear how extended resolution simulating clausal proofs can be effectively applied to resolution-based applications such as interpolation and abstraction refinement, making this an active area of research.

\subsection{DRUPing for Interpolants}
n \cite{DRUPing.for.interpolants}, the authors demonstrate how to leverage a DRUP clausal proof, as introduced in \cite{6679408} and explained in \ref{sec2.3}, for interpolation. In \cite{6679408}, two validation algorithms were proposed: backward and forward validation. Forward validation, which processes the proof from the leaves to the empty clause, is naturally suited for interpolation. However, because the DRUP clausal proof contains numerous irrelevant clauses—i.e., clauses that do not contribute to the derivation of the empty clause—forward validation can be inefficient. Therefore, \cite{6679408} recommends trimming the proof via backward validation, which eliminates all clauses not involved in deriving the empty clause. The approach in \cite{DRUPing.for.interpolants} involves trimming the DRUP proof to isolate the derivation of the empty clause, followed by replaying the trimmed proof and computing the interpolant on-the-fly.

\subsection{The Model Checker \avy}
\avy is a SAT-based model checker that combines interpolation and Property Directed Reachability (PDR)~\cite{avy}. It uses bounded model checking (BMC)~\cite{BMC} to search for a counterexample of length $k$. If such a counterexample does not exist, it extracts a sequence interpolant for the unsatisfiable BMC formula, and uses PDR to transform generalize the sequence interpolant and transform it to CNF. As a key part of the algorithm requires sequence interpolants, we use it in order to evaluate the DRUP interpolants framework implemented using \cadical.
